Entropy-Gradient Inversion: Moving Toward Internal Mechanism of Large Reasoning Models

The advancement of Large Reasoning Models (LRMs) has catalyzed a paradigm shift from reactive ``fast thinking'' text generation to systematic, step-by-step ``slow thinking'' reasoning, unlocking state-of-the-art performance in complex mathematical and logical tasks. However, the field faces \textit{the fundamental gap between token-level behavioral analysis and internal reasoning mechanisms, and the instability of reinforcement learning (RL) for reasoning optimization relying on costly external verifiers}. We identify and formally define \textbf{Entropy-Gradient Inversion}, a robust negative correlation between token entropy and logit gradients that acts as a definitive geometric fingerprint for LRM reasoning capability. Building on this, we propose \textbf{Correlation-Regularized Group Policy Optimization (CorR-PO)}, which embeds this inversion signature into RL reward regularization. Extensive experiments on various reasoning benchmarks across multiple model scales show CorR-PO consistently outperforms state-of-the-art baselines, confirming that stronger inversion directly correlates with superior reasoning performance.

==> multi_plots/correlation_samples_llama.tex <==
\begin{figure*}[t]
    \centering
    % --- Legend 部分 ---
      \centering
    \begin{minipage}{1\textwidth}
      \centering
    \includegraphics[width=0.55\textwidth]{figures/XAI_Samples_correlation/legend.pdf}
    \label{fig:XAI_Samples_correlation_legend}
  \end{minipage}
  % \vspace{-2em}
  \vskip\baselineskip % 换行
    % --- 第一行图片 ---
    \subfigure{
        \includegraphics[width=0.31\linewidth]{figures/XAI_Samples_correlation/entropy_logit_gradient_reasoning_samples_Llama_Combined.pdf}
        \label{fig:entropy_logit_gradient_reasoning_samples_Llama_Combined}
    } % 注意：这里建议保留 % 以防止意外空格
    \hfill  % 建议加上 \hfill 让左右两张图撑满一行，自动调整中间间距
    \subfigure{
        \includegraphics[width=0.31\linewidth]{figures/XAI_Samples_correlation/entropy_logit_gradient_safety_samples_Llama_Combined.pdf}
        \label{fig:entropy_logit_gradient_safety_samples_Llama_Combined}
    }
    \hfill  % 建议加上 \hfill 让左右两张图撑满一行，自动调整中间间距
    \subfigure{
        \includegraphics[width=0.31\linewidth]{figures/XAI_Samples_correlation/entropy_logit_gradient_base_samples_Llama_Combined.pdf}
        \label{fig:entropy_logit_gradient_base_samples_Llama_Combined}
    }
    
    % \vspace{-0.5em}
    \caption{\textbf{Spearman correlation between logit gradient nuclear norm and token entropy across different model types on Llama3.1-8B family}. The subfigures illustrate the correlation analysis conducted on different data distributions, specifically showing \textbf{Left}: \textit{Reasoning Samples}, \textbf{Middle}: \textit{Safety Samples}, and \textbf{Right}: \textit{Base Samples}. In each case, we evaluate three distinct model variants (Reasoning, Safety, and Base models) to demonstrate the consistent monotonic relationship between gradient sensitivity and predictive uncertainty across both diverse tasks and model alignment stages.}
    \label{fig:correlation_samples_Llama}
    % \vspace{-1.4em}
\end{figure*}
